Layout-your-3D: Controllable and Precise 3D Generation with 2D Blueprint

We present Layout-Your-3D, a framework that allows controllable and compositional 3D generation from text prompts. Existing text-to-3D methods often struggle to generate assets with plausible object interactions or require tedious optimization processes. To address these challenges, our approach leverages 2D layouts as a blueprint to facilitate precise and plausible control over 3D generation. Starting with a 2D layout provided by a user or generated from a text description, we first create a coarse 3D scene using a carefully designed initialization process based on efficient reconstruction models. To enforce coherent global 3D layouts and enhance the quality of instance appearances, we propose a collision-aware layout optimization process followed by instance-wise refinement. Experimental results demonstrate that Layout-Your-3D yields more reasonable and visually appealing compositional 3D assets while significantly reducing the time required for each prompt. Additionally, Layout-Your-3D can be easily applicable to downstream tasks, such as 3D editing and object insertion. Our project page is available at:https://colezwhy.github.io/layoutyour3d/

==> tables/layout_numerical.tex <==
\begin{table}[htp]
\centering
\scriptsize
\renewcommand\arraystretch{1.}
\vspace{-.2in}
\caption{Comparison of different foundation models used when rectifying rotation $r_i$ in the Coarse 3D Generation stage.}
\vspace{.1in}
\begin{tabular}{l | c c}
\toprule
Model & CLIP  & DINOv2 &\\
\midrule
Average error & & \\ 
\bottomrule
\end{tabular}
\label{tab: rotation}
\vspace{-.1in}
\end{table}

